What to tell when? -- Information Provision as a Game

Constantly informing systems (CIS), that is technical systems that provide us with information over a long period of time, face the challenge of providing us with helpful information. The information base of a human model changes over time but also his mood and his ability to accept information. An information provision strategy should hence take such aspects into account. In this paper, we describe our vision of an approach to aid the design of CIS. We envision using psychological models of the human mind and emotions in an information provision game. Its analysis gives comparative insights into design variants.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Farrell, M. Luckcuck, M. Schwammberger, and\\ M. Gleirscher (Eds): Fifth International Workshop on \\Formal Methods for Autonomous Systems (FMAS 2023)\\
EPTCS 395, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.395.1}{10.4204/EPTCS.395.1}}
\pdfoutput=1

